BRAIn: Bayesian Reward-conditioned Amortized Inference for natural language generation from feedback

Distribution matching methods for language model alignment such as Generation with Distributional Control (GDC) and Distributional Policy Gradient (DPG) have not received the same level of attention in reinforcement learning from human feedback (RLHF) as contrastive methods such as Sequence Likelihood Calibration (SLiC), Direct Preference Optimization (DPO) and its variants. We identify high variance of the gradient estimate as the primary reason for the lack of success of these methods and propose a self-normalized baseline to reduce the variance. We further generalize the target distribution in DPG, GDC and DPO by using Bayes' rule to define the reward-conditioned posterior. The resulting approach, referred to as BRAIn - Bayesian Reward-conditioned Amortized Inference acts as a bridge between distribution matching methods and DPO and significantly outperforms prior art in summarization and Antropic HH tasks.

==> icml2024/new_commands_and_packages.tex <==
\usepackage{bbm}
\usepackage{booktabs} 
\usepackage{wrapfig}
\usepackage{comment}
\usepackage{cleveref}
\usepackage[nounderscore]{syntax}


\usepackage{thmtools,thm-restate}

\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{assumption}[theorem]{Assumption}
\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}

%\newtheorem{theorem}{Theorem}
%\newtheorem{example}{Example}
%\newtheorem{lemma}[theorem]{Lemma}




\newcommand{\etal}{\mbox{\it et al.}}
\newcommand{\etc}{\mbox{\it etc.}}
\newcommand{\eg}{\mbox{\it e.g.}}
\newcommand{\ie}{\mbox{\it i.e.}}
\newcommand{\cf}{\mbox{\it cf.}}
\newcommand{\Eg}{\mbox{\it E.g.}}
\newcommand{\Ie}{\mbox{\it I.e.}}
\newcommand{\wrt}{\mbox{\it w.r.t.}}
\newcommand{\?}{\mbox{?}}
\newcommand{\myqed}{\blacksquare}
\newcommand{\viz}{\mbox{\it viz.}}


\newcommand{\shortname}{\textsc{BRAIn}}
\newcommand{\longname}{\textbf{B}ayesian \textbf{R}eward-conditioned \textbf{A}mortized \textbf{In}ference}

\newcommand{\mle}{\theta^*}
\newcommand{\bigprob}{\mathbb{P}}
\newcommand{\yset}{\mathcal{Y}}


\newcommand{\RL}{RL }
\newcommand{\KL}{D_{KL} }
\newcommand{\KLnorm}{D_{n}^{q'}}
\newcommand{\inp}{x}
\newcommand{\outp}{y}
\newcommand{\outpp}{{\outp}}
\newcommand{\outpvec}{\mathbf{y}}
\newcommand{\outppvec}{{\mathbf{y}}}
\newcommand{\maxlength}{L_{max}}
\newcommand{\rewardrv}{G}
\newcommand{\goodness}{g}
\newcommand{\ppolicy}{q_{\theta}}
\newcommand{\pposterior}{p}
\newcommand{\pproposal}{q'}
\newcommand{\entropy}{\mathcal{H}}
\newcommand{\boutp}{\bar{\outp}}
\newcommand{\dposft}{DPO-sft}
\newcommand{\dpoiw}{DPO-sft + IW}
\newcommand{\dpoiwn}{DPO-sft + IW + n}
\newcommand{\rewardpprob}{p(\rewardrv=1|\inp, \outp)}
\newcommand{\alphahatyx}{\hat{\alpha}_{Y_x}}
\newcommand{\betahatthetayx}{\hat{\beta}_{Y_x}}

\newcommand{\betatheta}[1]{\beta_{#1}(\theta)}
\newcommand{\alphay}[1]{\alpha_{\outp_{#1}}}
\newcommand{\alphahaty}[1]{\hat{\alpha}_{\outp_{#1}}}
\newcommand{\betathetay}[1]{\beta_{\outp_{#1}}}
\newcommand{\betahatthetay}[1]{\hat{\beta}_{\outp_{#1}}}
%\newcommand{\betathetay}[1]{\beta_{\outp_{#1}}(\theta)}
%\newcommand{\betahatthetay}[1]{\hat{\beta}_{\outp_{#1}}(\theta)}


\newcommand{\rewardfn}[1]{r(\inp,{#1})}
\newcommand{\prior}[1]{p({#1}|\inp)}
\newcommand{\posterior}[1]{p({#1} | \inp, \rewardrv=1)}
\newcommand{\policy}[1]{q_{\theta}({#1} | \inp)}

\newcommand{\proposal}[1]{q'({#1} | \inp)}
\newcommand{\reference}[1]{p_{\text{ref}}({#1} | \inp)}
\newcommand{\optimal}[1]{p^{*}({#1} | \inp)}

\newcommand{\rewardprob}[1]{p(\rewardrv=1|{#1},\inp)}
\newcommand{\rewardprobx}{p(\rewardrv=1| \inp)}
\newcommand{\pnorm}[1]{p_n({#1}|\inp, \rewardrv=1)}
\newcommand{\qnorm}[1]{q_n({#1}|\inp)}


\newcommand{\expectation}{\mathbb{E}}
\newcommand{\loss}{\mathcal{L}_x(\theta)}
\newcommand{\lossestimate}{\hat{\mathcal{L}}_x(\theta)}
\newcommand{\multiexpectation}{\mathbb{E}_{\substack{\outp_i \sim \proposal{\outp} \\ 1 \leq i \leq n}}}
\newcommand{\multiexpectationdpo}{\mathbb{E}_{\substack{\outp_1, \outp_2 \sim \prior{\outp} }}}





==> icml2024/sections/experiments_31stJan1030am.tex <==
\section{Experimental Results}
\subsection{Objectives}
This section evaluates \shortname's performance in natural language generation from feedback, focusing on:
1) Performance comparison of \shortname\ with state-of-the-art methods.
2) Investigating how baseline subtraction affects \shortname's performance.
3) Assessing the impact of mis-specifying the reward model $\rewardpprob$ on \shortname.
4) Examining the effect of varying output sample numbers per input on \shortname.
5) Analyzing the performance gap between  \dposft and \shortname, and potential bridging strategies.

\subsection{Tasks}
We explore three natural language generation tasks - summarization, multi-turn dialog and sentiment-controlled generation. For the first two tasks, the underlying reward model is a preference model trained using Bradley-Terry assumptions. The third task uses a classifier trained using logistic regression as the reward model. For the sake of reproducibility, we use models publicly available on huggingface as our base model (prior) and reward function in all the three tasks. 

\textbf{Summarization:} 

\textbf{Multi-turn dialog:}

\textbf{Sentiment-controlled generation:}
\subsection{Evaluation}
We evaluate our models on three tasks using the win-rate against the gold response in the test set as the evaluation criterion. To compute the win-rate, we employ three approaches:

\textbf{Train Reward Function:} We calculate the rewards for both the gold and generated outputs on the test set using the reward function employed during training. The output with the higher reward is deemed the winner. This experiment indicates the effectiveness of each approach in maximizing the specified reward function.

\textbf{Independent Reward Model:} We utilize an independent reward model\footnote{\url{https://huggingface.co/OpenAssistant/oasst-rm-2-pythia-6.9b-epoch-1}} not used during training for evaluation, demonstrating the cross-reward generalization capability of each approach. 

\textbf{Large Language Model Evaluation:} Outputs are evaluated using powerful large language models (LLMs) such as Mixtral-7B\footnote{\url{https://huggingface.co/mistralai/Mixtral-8x7B-Instruct-v0.1}}~\cite{jiang2023mistral} and GPT-4~\cite{achiam2023gpt}. These LLMs are asked to choose the preferred output. The specific prompt used for this evaluation is detailed in the appendix.

\subsection{Baselines}
We compare the performance of our model against several state-of-the-art baselines:

\textbf{DPO:} The DPO objective is directly trained on preference pairs. We set the temperature parameter to $1$.

\textbf{\dposft:} For \dposft, we first generate samples from the base policy, and then compute the reward for the generated samples. The generated samples for a given input are grouped in pairs and used for training. The temperature parameter is set to $1$.

\textbf{SLiC-HF:} For SLiC-HF, we follow a similar setting as \dposft. We use a margin of $1.0$ for the margin-loss. The regularization weight is also set to $1$.

\textbf{RSO:} As shown in \cite{liu2023rso}, RSO can be thought of as \dposft with hinge-loss, where the samples are obtained via rejection sampling. As suggested in the paper, we set $\beta = 0.5$ and $\gamma = 0.05$.

\textbf{QUARK:} \gcom{Waiting for the results}

\subsection{Results}

\subsubsection{Performance comparison against baselines:}
We train each model that uses pairwise data (DPO, \dposft\ , SLiC and RSO) for a total of $10000$ steps with a batch size of $32$ preference pairs. The model is evaluated after every $1000$ steps and the best model is selected based on the win rate against gold response on the cross-validation set.

\input{icml2024/tables/performance_comparison}

\subsubsection{Bridging the gap between \dposft and \shortname}
As shown in the previous section, \shortname does a better job at optimizing the reward function than \dposft.
In Section~\ref{sec:dpo_sft}, we observed that \dposft can be viewed as a special case of \shortname when only 2 outputs are sampled at a time from the prior $\prior{\outp}$ and the corresponding importance weights are discretized to be either $0$ or $1$. 
Hence, this suggests that we should be able to bridge the gap between \shortname and \dposft by lifting some of the restrictions. To achieve this, we first add the importance weights to the DPO objective to get \eqref{eq:dpo_sft_iw}. Next, we increase the number of samples in the importance-weighted DPO objective from $2$ to $32$ to get the objective mentioned in \eqref{eq:dpo_sft_iw_n}. Finally, using a mixture proposal distribution as defined in Section \ref{sec:proposal} closes the gap. The results for Anthropic HH are given in Table~\ref{tab:dpo_brain_gap}. Note that all the models in table use $32$ output samples per prompt during training. 
\input{icml2024/tables/dpo_brain_gap}





Next, we allow any finite number of samples in the \dpoiw objective as shown below.


==> icml2024/sections/introduction_backup.tex <==
\section{Introduction}
\label{sec:intro}

% \textbf{Motivation}:
% \begin{enumerate}
%     \item Given a reward function and a base generator, approaches for learning from feedback - PPO-RLHF, SLiC, RRHF either treat the problem as expected maximisation of the reward function or contrast between high reward and low-reward samples. The models are also regularized to be close to the base generator.
%     \item None of these approaches account for the underlying distributions that these reward functions correspond to. For instance, if the Bradley-Terry model was parametrized differently (say, $P(yi>yj|x)) = r(x,y_i)/r(x, y_i) + r(x, y_j)$, the distributions that the reward functions correspond to will be different. However, PPO, SLiC and RRHF would still treat the reward functions similarly.
%     \item The exception is DPO. DPO says that instead of using human annotations for learning a reward function, we can directly use those human annotations for training our policy (Lets call this model as DPO-fixed). Empirically, however, it has been observed that DPO performs better when the human annotations are used for learning a reward function and the reward function is then used to label the samples generated by a base model. Lets call this DPO-base.  The derivation of DPO objective doesn't explain why it is better to use samples from base policy than the ones that were used for human annotation. (Mathematically, write the two formulations of DPO, one has human-annotated samples, the other has samples from the base model and uses a reward function)
%     \item A limitation of DPO is that it assumes that for a given reward function, reward maximization with KL-control (RM-KL) is the best thing to do, finds the form of the optimal policy in  RM-KL and plugs it into the reward model. However, RM-KL ignores the underlying distribution captured by the reward function. Instead, we propose to use Bayes's rule to incorporate the distributions captured by the reward functions into our policy.  We then use amortized inference (cite VAE) to mimic the resultant posterior by minimizing the KL divergence between the inference network and the posterior. The resultant approach is termed as \shortname (Bayesian Reward-conditioned Amortized Inference).
%     \item To reduce the variance of the gradient of our objective, we propose baselines that keep the expected gradient consistent.
%     \item Next, we derive the form of the posterior for absolute reward model, Bradley-Terry reward model and Plackett-Luce Model. We show that for Bradley-Terry reward models, the posterior corresponds to the PPO-optimal policy.
%     \item As a special case of \shortname we also derive the DPO formulation that uses the reward function to label samples from the base policy. This justifies the success of DPO-sft over DPO-fixed since DPO-sft follows from Bayes' rule. We show that DPO-sft can further be improved by explicitly incorporating the reward function in the objective rather than using it for just ranking the samples.
%     \item We show that \shortname outperforms all existing approaches for RLHF on summarization and AnthropicHH
%     \item We study the dependence of \shortname's performance  on the number of sampling used for approximating the gradient
% \end{enumerate}


Reinforcement Learning from Human Feedback (RLHF) has emerged as a pivotal technique to fine-tune Large Language Models (LLMs) into conversational agents that obey pre-defined human preferences \cite{ouyang2022training, bai2022training, openai2023gpt4, touvron2023llama}. This process involves collecting a dataset of human preferences and using it to align a Supervised Fine-Tuned (SFT) model to human preferences. 
 
%This \textit{alignment} process involves the collection of a human preferences dataset and both Supervised Fine Tuning (SFT) and RL training stages to adapt the model to user preferences. 
%\ycom{
%Typically, LLMs are first pre-trained on a very large corpus of text for the next word prediction task, followed by supervised fine-tuning (SFT) on a diverse set of instruction-following datasets \cite{shen2023flanmoe, chung2022scaling}.
%The next step involves aligning an SFT model to human preferences in which we first collect a human-preference dataset,
%train a reward model using the collected dataset, and finally
%fine-tune the SFT model so that it prefers outputs with high reward.
%}

Proximal Policy Optimization (PPO) RLHF \cite{ziegler2019pporlhf}, has been instrumental in the development of groundbreaking models such as GPT-3.5 \cite{ouyang2022training,ye2023comprehensive} and GPT-4 \cite{openai2023gpt4} among others. 
%This RL technique trains a separate Reward Model (RM) to discriminate model outputs that follow user preferences and optimizes an initial policy to maximize the expected reward, while regularizing it to not diverge too much from that policy. 
This RL technique trains a separate Reward Model (RM) to discriminate outputs that follow human preferences.
The RM is then used to train a policy that maximizes the expected reward while regularizing it to not diverge too much from the SFT model. 
Despite its clear success, PPO has been lately displaced by offline-RL contrastive techniques that are more scalable but do not make full use of a separate RM. %Direct Preference Optimization (DPO) \cite{rafailov2023direct} is one such technique which is currently the de-facto method used to align high-performing models such as Zephyr \cite{tunstall2023zephyr}, Tulu \cite{ivison2023camels} or Neural-Chat. % While PPO uses the reward score during train, most contrastive techniques use RM only for ranking the outputs.
% \footnote{DPO does not use a separate RM. However, its form does depend on a reward model choice (Bradley-Terry/Plackett-Luce).}
%but that limit the way in which an RM can be used. 
Techniques like Likelihood Calibration (SLiC) \cite{zhao2023slic} or Rank Responses (RR)HF \cite{yuan2023rrhf} only keep ranking information from a RM. On the other hand, techniques like Direct Preference Optimization (DPO) \cite{rafailov2023direct}, which is currently the de-facto method used to align high-performing models such as Zephyr \cite{tunstall2023zephyr}, Tulu \cite{ivison2023camels} or Neural-Chat\footnotemark,  do not even have a separate RM. %\footnotemark\footnotetext{Note, however, that DPO's form does depend on a reward model choice (Bradley-Terry/Plackett-Luce).}. 

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{icml2024/figures/brain-intro.pdf}
    \caption{Two examples used for training alignment algorithms with different reward situations: one where the rewards have a big gap, and another where the gap is smaller.}
    \label{fig:intro}
\end{figure} 

% disentangle the below two items:
% the need for separate RM 
    % Does any approach warm start RM with additional data - citation required
    % cite RSO, SLiC for RM can be used to label new data
% motivate that reward magnitudes have valuable information and that is unused by the contrastive approaches.

%Arguably, there are inherent advantages to having a separate RM. It can be warm-started with additional data not suited for LLM training \cite{roit-etal-2023-factually}, leading to complementary knowledge to that of the conversational agent. Further, a separate RM can be used to label new data by generating multiple outputs from SFT model. 

Rewards obtained using an RM trained on human preference convey additional fine-grained information about the outputs. Consider the two cases in \Cref{fig:intro}. In the first example, one output is clearly better than the other. Whereas, in the second example, both outputs are almost equally good.
Therefore the first example is more important for alignment than the second example. The gap in reward scores captures this importance. 
%The first example has a big gap indicating is important to learn to align to the output with a higher reward, while it is not so crucial to align the second example to the higher reward output.
Recent alignment models such SLiC, RRHF, and DPO ignore this crucial fine-grained RM information.

% Unfortunately, all recent alignment algorithms are limited in how they use this information effectively. They ignore the magnitude of the score assigned by the separate RM and rely only on the ranking of the outputs.

% ARE WE ARGUING THIS IS SUBOPTIMAL?
%We argue that this is suboptimal. 

%To see this, consider the two examples in \cref{fig:intro}. Both answers are equally good in the second example, whereas in the first example, the latter answer is clearly wrong. However, the ranking-based algorithms and DPO will ignore this information conveyed by the actual scores and treat both examples in the same way.

In this work, we develop an alignment method that returns to a more explicit use of RMs but retains the scalability of recent techniques. 
For this, we propose \shortname: \longname.
\shortname~starts from a different principle than PPO or DPO, which focuses on regularized reward maximization. 
Here we aim to distill the reward-conditioned posterior $\posterior{\outp}$, understood as conditioning the prior distribution $p(y \mid x)$ (SFT model) to obtain only outputs that are deemed good ($G=1$).
%\ycom{Next line is not clear.}
%Rather than parametrizing this distribution directly, which would require specific training data, \shortname~distills it into a single amortized policy parametrized by an LLM.
%\ycom{
%\begin{comment}
Instead of training a reward-conditioned model, such as Quark \cite{lu2022quark}, that first takes both prompt $\inp$ and quantized reward as input while training and then freezes reward to a high value during inference, \shortname\ directly distills the posterior distribution with fixed $G=1$ into an amortized policy parameterized by an LLM.
%\end{comment}
%}
The connection with RMs is attained by decomposing the posterior via Bayes theorem and parametrizing the likelihood, a \textbf{G}oodness model $\rewardprob{\outp}$, with the reward function. To sample from the posterior, \shortname~leverages self-normalised importance sampling ratios \cite{owen2013monte}. To reduce the variance of the gradient \cite{schulman2017proximal,ziegler2019pporlhf,sutton1999policy}, we propose a novel self-normalized baseline and prove that the baseline-subtracted gradient estimate is an unbiased estimator of a divergence measure that we refer to as self-normalized KL divergence.

%As we will show, this relation is also contingent on the underlying RM, such as Bradley-Terry or Logistic Regression, assumed during the reward function training and leads to an interesting connection with DPO, with potential enhacements.

%We want the finetuned language model to assign a high probability to `good' outputs ($\rewardrv=1$). One such distribution is the reward--conditioned posterior $\posterior{\outp}$ that conditions on the output being good.
%\gcom{
%Should we reword? Ideally, the posterior should be defined only after defining prior and likelihood.
%}
%With Bayes' rule, we represent the desired posterior using the goodness model $\rewardprob{\outp}$ as likelihood and the pre-trained LLM as a prior $\prior{\outp}$.
%Since we can't sample directly from the posterior policy, we train an amortized inference network (a causal LLM  in our case) to mimic the behaviour of the reward-conditioned posterior policy by minimizing the KL divergence between the posterior and the inference network. We call this as \shortname\ objective.
%We empirically show that explicitly incorporating the reward into the training objective significantly improves performance.

%To empirically estimate the KL divergence, we sample many outputs from an easy-to-sample proposal distribution

% TODO: reuse later
%Next, we derive the exact form of the \shortname\ objective for Bradley-Terry and Logistic Regression reward models by showing the connection between our goodness model and the reward function.

% TODO: Reuse later
%\ycom{Feedback from Sachin: para on dpo is complicated.. Simplify}
%Direct Preference Optimization \cite{rafailov2023direct} is one of the recently proposed approaches that circumvent training the reward function completely and finetunes the LLM directly using the preference triplets $(\inp, \outp_w, \outp_{\ell})$ (winner $\outp_w$ is preferred over lower $\outp_\ell$), typically used to train the reward model.
%Even though they do not train a reward model, interestingly, their training objective is derived assuming a specific reward model, \eg, Bredley-Terry.
%Under the assumption that the training outputs $\outp_w$ and $\outp_\ell$ are sampled from the supervised fine-tuned model (prior policy), we prove that DPO objective is a special case of \shortname.  

In our experiments on TL;DR summarization \cite{stiennon2020learning,volske2017tldr} and AntropicHH \cite{bai2022training},
%, and positive sentiment completion \cite{sentiment_task} tasks, 
\shortname\ establishes a new state-of-the-art by significantly outperforming existing s-o-t-a RL method DPO \cite{rafailov2023direct}.
In addition, we bridge the gap between \shortname\ and DPO by careful augmentation of DPO objective in two ways. Specifically, we incorporate:
1) multiple outputs for a given input prompt, and 2) reward as an importance weight in the DPO objective. 

Overall, we make the following contributions:

% \begin{compactenum}
% \item To align an LLM to user preferences using feedback from a given reward function, we introduce \shortname: a framework with a novel training objective and a novel baseline for variance reduction. Unlike existing methods, our objective takes the reward values into account while fine-tuning.

% \item We theoretically prove that our proposed gradient estimate is an unbiased estimator of a form of divergence measure that we refer to as self-normalized KL divergence. \rcom{That
% asymptotically converges to the true objective} 
% \item  We derive the exact form of our objective under Bradley-Terry, and Logistic Regression reward models.
% \item We derive DPO as a special case of our objective when training samples are drawn from the SFT policy.
% \item Finally, we empirically substantiate our claims by experimenting on two natural language generation tasks and comparing \shortname\ against existing s-o-t-a alignment methods.
%\end{compactenum}

\begin{compactenum}
\item We propose \shortname, a novel algorithm to align an LLM to human-preferences. Unlike existing ranking-based methods, \shortname\ incorporates fine-grained reward scores while training. \shortname\ uses a novel self-normalized baseline for variance reduction of the proposed gradient estimate.
\item We theoretically prove that the proposed gradient estimate is an unbiased estimator of a modified form of KL divergence that we name \shortname~objective.
\item We derive the exact form of the \shortname~objective under Bradley-Terry preference model assumption. We also show DPO can be derived as a special case of the \shortname~objective.
\item Finally, we empirically substantiate our claims by experimenting on two natural language generation tasks.
%\item Departing from a distribution matching approach, we derive the \shortname~gradient update rule, which leverages self-normalized importance sampling and a novel variance reduction baseline.
%\item We prove that this gradient update rule is an unbiased estimator of a modified form of KL divergence that we name \shortname~objective.
%\item We show DPO can be derived as a special case of the \shortname~objective, where fine-grained information in the reward is discarded.
%\item We derive the exact form of the \shortname~objective under Bradley-Terry preference model assumption.
%\item Finally, we empirically substantiate our claims by experimenting on two natural language generation tasks. Ablation analysis confirms limitations in DPO and shows large gains over this method when using the full \shortname~update rule
\end{compactenum}

%In this paper, we show that incorporating the reward explicitly into the training objective can result in significant improvement in performance. To achieve that, we use the underlying probability model captured by the reward function (for instance, Bradley-Terry model or Logistic Regression model) to define a \textit{Goodness} model. Treating the Goodness model as likelihood and the base policy (this is often a supervised finetuned LLM) as prior, we use Bayes' rule to obtain the reward-conditioned posterior. Since it is difficult to sample from the posterior policy, we train an amortized inference network (a causal LLM, in our case) to mimic the behavior of the reward-conditioned posterior policy. The resultant approach is referred to as \textbf{B}ayesian \textbf{R}eward-conditioned \textbf{A}mortized \textbf{In}ference (or \shortname). 

%As has been common in policy gradient-based approaches for RL~\cite{schulman2017proximal,ziegler2019pporlhf,sutton1999policy}, we show that variance reduction is the key to achieve reasonable performance with \shortname. Hence, we incorporate two tricks to reduce variance of the gradient of objective - self-normalization and subtracting an appropriate baseline. Specifically, we propose a self-normalized baseline and show that the baseline-subtracted gradient estimator is a statistically consistent estimator for the gradient of \shortname.

%We derive the exact form of the objective for Bradley-Terry, Plackett-Luce and Logistic Regression reward models. As a special case of \shortname, we derive the DPO objective where the samples for training come from the base policy, thereby connecting \shortname with DPO. In our experiments section, we compare \shortname against state-of-the-art approaches for reinforcement learning in LLMs - SLiC~\cite{zhao2023slic}, DPO~\cite{rafailov2023direct} and Quark~\cite{lu2022quark} and show that \shortname outperforms these approaches on several evaluation metrics. In our ablation, we bridge the gap between DPO and \shortname by extending the DPO objective in two ways: 1) Incorporating multiple outputs for a given input prompt in the DPO objective 2) Incorporating the reward as an importance weight in the DPO objective. We show that each of these steps result in performance improvement for DPO.









\begin{comment}
% In this paper, we propose a novel approach to reinforcement learning in LLMs, which we term ``reward conditioned distillation." Our method leverages the reward function and the base LLM to define a posterior distribution over the outputs for a given input. Due to the complexity of directly sampling from this posterior distribution, we distil it into a trainable policy. This is achieved by minimizing the Kullback-Leibler (KL) divergence between the posterior distribution and the trainable policy, thereby effectively translating the reward information into the model's learning process.

% A key aspect of our approach is the distinction between optimizing reverse KL divergence, which aligns with the traditional PPO-RLHF objective, and forward KL divergence. 
% \ycom{Maybe rephrase the above line as: Unlike PPO-RLHF which focuses on reverse KL divergence, our technique optimizes forward KL divergence.}
% The traditional on-policy method, while effective, comes with several drawbacks, including sample inefficiency and challenges in exploring the output space. By contrast, when optimizing forward KL divergence, we transition to an off-policy method of reinforcement learning. This shift not only addresses some of the limitations of on-policy methods but also generalizes contrastive approaches such as Direct Policy Optimization (DPO). Our method is unique in that it models the probabilities of multiple outputs within a single objective, providing a more comprehensive and nuanced approach to reinforcement learning in LLMs.

% Through this paper, we aim to introduce and validate our proposed reward distillation approach, highlighting its potential to redefine the boundaries of reinforcement learning in large language models and pave the way for more efficient, robust, and versatile AI systems.
\end{comment}




==> icml2024/sections/technique_25thJan.tex <==
\section{Problem Formulation}

\section{Approach}

\textbf{Bayesian reformulation:}
We first use Bayes' rule to represent the reward--conditioned posterior as:
\begin{equation}\label{eq:posterior}
    \base(\outp \mid \inp, \rewardrv=1) =  \frac{\base(\outp \mid \inp) \rewardprob(\rewardrv=1 \mid \outp, \inp)}{\sum_{\bar{\outp} \in \yset}\base(\bar{\outp}|\inp)\rewardprob(\rewardrv=1 \mid \bar{\outp}, \inp)}
\end{equation}
Using the law of total probability, we can see that the denominator in the above equation represents $\rewardprob(\rewardrv=1|\inp)$.
Intuitively, it captures the average goodness over all output samples for a given input $\inp$.



\section{Approach}
First, we define our problem of Bayesian reward conditioned distillation by specifying the prior, likelihood and the posterior. We provide an importance weighted approximation to the posterior and suggest a baseline to reduce variance in the subsequent sections. 

\subsection{Bayesian Reward Conditioned Distillation}
 Let $x$ be an input prompt and $\yset$ be the set of all output sequences with maximum length $L_{max}$. We assume that we are provided a base model $p(y|x)$ for generating outputs conditioned on a given input prompt. In our Bayesian framework, this base model corresponds to the prior distribution over the outputs. 
 
 Given an input $x$ and and output $y \in \yset$, we encode the absolute (or non-relative) measure of goodness of $y$ using a binary random variable $R_{xy}$. Specifically, for a given prompt $x$, the goodness of the output $y$ is captured in the probability $p(R_{xy}=1|x,y)$. In Section~\ref{sec:btm}, we show how this probability can be computed for absolute as well as relative reward models (such as Bradley-Terry preference models).
 
Given the prior $p(y \mid x)$ and the stochastic reward model $p(R_{xy}=1|x,y)$, the reward-conditioned model corresponds to the posterior and can be expressed using Bayes' rule 
\begin{equation}\label{eq:posterior}
    p(y \mid x, R_{xy}=1) =  \frac{p(y \mid x) p(R_{xy}=1 \mid y,x)}{\sum_{\bar{y} \in \yset}p(\bar{y}|x)p(R_{x\bar{y}}=1 \mid \bar{y}, x)}
\end{equation}

For notational convenience, we represent the denominator of the above equation as $p(R_x=1|x)$. Intuitively, $p(R_x=1|x)$ represents the probability that an average sample from the base model $p(y|x)$ is good.

We are interested in sampling from $p(y \mid x, R_{xy}=1)$, that is, samples with high reward. An obvious solution is to sample from $p(y \mid x)$ and keep rejecting the samples until a high value of the ratio $\frac{p(R_{xy}=1 \mid y,x)}{p(R_{x}=1 \mid x)}$ is obtained. 

Despite its simplicity, rejection sampling is expensive. Hence, in this work, we propose to learn a distribution that can mimic sampling from the posterior without the computation overhead of rejection sampling. 



To achieve this, we propose to minimize the KL-divergence between the posterior distribution $p(y \mid x,R_{xy}=1)$ and a parameterized autoregressive model $q_\theta(y \mid x)$. This is equivalent to maximizing the objective $\mathcal{L}_x$ below:
\begin{align}
    \mathcal{L}_x(\theta) &= - E_{p(y \mid x, R_{xy}=1)} \left[ \log \frac{p(y \mid x) p(R_{xy}=1 \mid y,x)}{p(R_{x}=1 \mid x)q_\theta(y \mid x)} \right]
\end{align}
By collecting all the constant terms with respect to $\theta$ in $C$, the objective can be written as
\begin{align}\label{eq:objective}
    \mathcal{L}_x(\theta) &=  E_{p(y \mid x, R_{xy}=1)} \left[ \log q_\theta(y \mid x) \right] +C\,,
\end{align}

% Using \eqref{Bayes}, the expectation with respect to the posterior can be replaced by an expectation with respect to the base model $p(y \mid x)$
% \begin{align}\label{importance}
%     \mathcal{L}_x &= \sum_{r \in \{0,1\}} E_{p(y \mid x)} \left[\frac{p(r \mid y,x)}{p(r \mid x)}\right]  \log q_\theta(y \mid x,r) 
% \end{align}
Henceforth, the constant $C$ will be omitted in subsequent formulations of the objective $\mathcal{L}_x$.

\subsection{Approximating the objective with importance sampling}\label{sec:approx_is}
Since $p(y|x,R_{xy}=1)$ defined in \eqref{eq:posterior} doesn't allow for direct sampling, we use importance sampling to estimate the objective in~\eqref{eq:objective}. Specifically, let $q'(y|x)$ be a proposal distribution from which we can more easily sample. The key is to choose $q'(y|x)$ such that it is sufficiently similar to $p(y|x,R_{xy}=1)$, to ensure efficient sampling. Using self-normalized importance sampling (Chapter 9 in \cite{owen2013monte}), the objective can be approximated using samples from the proposal distribution $q'(y|x)$ as follows:
\begin{align}\label{eq:approx_is}
&\hat{\mathcal{L}_x}(\theta) = \frac{\sum_{i=1}^n \alpha_{i} \log q_\theta(y_i \mid x)}{\sum_{j=1}^n \alpha_{j}} \\
&\text{ where } y_i \sim q'(y|x) \text{ and } \\& \alpha_{i} = \left(\frac{p(y_i \mid x)}{q'(y_i \mid x)}\right) p(R_{xy_i}=1| y_i, x)
\text{, } 1\le i \le n \label{eq:alpha}
\end{align}
The weights $\alpha_{i}$ are referred to as importance weights and correspond to the ratio of the probability of the sampled point $y_i$ under the posterior  and proposal distribution respectively. A straightforward derivation of the above equation is shown in the Appendix. Importantly, self-normalization helps us to get rid of the normalization constant in the computation of importance weights albeit at the cost of introducing bias in the objective.




\subsection{Baseline subtraction}
The gradient of the posterior distillation objective with respect to the parameters $\theta$ defined in \eqref{eq:objective} can be written as
\begin{equation}
    \nabla_\theta \mathcal{L}_x(\theta) = E_{p(y|x, R_{xy}=1)} \nabla_\theta \log q_\theta(y|x)
\end{equation}

To obtain a baseline for the above expected gradient, we first note the following well-known result:
\begin{align}
     E_{q_\theta(y|x)} &  \nabla_\theta \log q_\theta(y|x) = 0
\end{align}
A proof of the same is given in the appendix.
% \begin{align}
%     E_{q_\theta(y|x)} &  \nabla_\theta \log q_\theta(y|x) = \sum_{y \in \yset} q_\theta(y|x) \frac{\nabla_\theta q_\theta(y|x)} {q_\theta(y|x)} \\
%     & = \sum_{y\in \yset} \nabla_\theta q_\theta(y|x) = \nabla_\theta \sum_{y\in \yset} q_\theta(y|x) = \nabla_\theta 1 = 0
% \end{align}
Thus, the gradient of the objective can be rewritten as
\begin{align}
    \nabla_\theta \mathcal{L}_x(\theta) =& E_{p(y|x, R_{xy}=1)} \nabla_\theta \log q_\theta(y|x) - \\& E_{q_\theta(y|x)} \nabla_\theta \log q_\theta(y|x)
\end{align}
Next, given the proposal distribution $q'(y|x)$, we approximate the two expectations in the above equation by self-normalized importance sampling making sure that the same set of samples are used in both the approximations. 
\begin{align}\label{eq:approx_is_bs}
    \nabla_\theta \hat{\mathcal{L}_x}(\theta) = & \frac{\sum_{i=1}^n \alpha_i \nabla_\theta \log q_\theta(y_i|x)}{\sum_{j=1}^n \alpha_j } - \\
    &\frac{\sum_{i=1}^n \beta_i \nabla_\theta \log q_\theta(y_i|x)}{\sum_{j=1}^n \beta_j } \notag\\
    =& \sum_{i=1}^n \left(\frac{\alpha_i}{\sum_{j=1}^n \alpha_j} - \frac{\beta_i}{\sum_{j=1}^n \beta_j}\right) \nabla_\theta \log q_\theta(y_i|x)\,, \\
    \text{ where } & y_i \sim q'(y|x) \text{, } \alpha_{i} = \left(\frac{p(y_i \mid x)}{q'(y_i \mid x)}\right) p(R_{xy_i}=1| y_i, x)\\
    &\text{ and } \beta_i = \frac{q_\theta(y_i|x)}{q'(y_i|x)} \text{, } 1\le i \le n \notag
\end{align}
The $\alpha_i$'s are the same importance weights that we defined in Section~\ref{sec:approx_is} while the $\beta_i$'s correspond to the importance weights of the baseline. Intuitively, we can make the following observations:
\begin{itemize}
    \item The original importance-sampling objective defined in \eqref{eq:approx_is} assigned positive weight to the log-probability of each output $y_i$ irrespective of the reward.
    \item Since the posterior $\propto p(y|x)p(R_{xy}=1|y,x)$, the baseline-subtracted objective \eqref{eq:approx_is_bs} assigns positive weight to those $y_i$'s where the self-normalized trainable policy $q_\theta(y|x)$ assigns lower probability to the output than the self-normalized posterior, thus increasing $q_\theta$ for such outputs.
    \item For outputs where the policy assigns higher probability than the posterior, the weights in \eqref{eq:approx_is_bs} are negative, thereby decreasing $q_\theta$ for such outputs.
\end{itemize}

In our experiments, we show that subtracting this baseline results in tremendous improvement in performance. We hypothesize that the baseline allows the model to focus on features that are distinctive of high-reward outputs as compared to the lower reward ones..

\subsection{Bradley-Terry Preference Model for LLMs}\label{sec:btm}
Let $y_1, \ldots, y_n$ be a set of items and $p_1, \ldots, p_n$ be their corresponding weights. The weights represent an absolute measure of the goodness of the individual items. Given two items from the set $y_i$ and $y_j$, the probability of preferring $y_i$ over $y_j$ in a Bradley-Terry preference model is defined as
\begin{equation}
    \bigprob(y_i \succ y_j) = \frac{p_i}{p_i + p_j}
\end{equation} 

In the context of language models, $y_i$'s are often sequences generated conditioned on an input prompt $x$. Let $\yset$ be the set of all output sequences with maximum length $L_{max}$. Given an input $x$ and and output $y \in \yset$, we encode the absolute measure of goodness of $y$ using a binary random variable $R_{xy}$. Specifically, for a given prompt $x$, the goodness of the output $y$ is captured in the probability $p(R_{xy}=1|x,y)$. Thus, we define a Bradley-Terry model where the probability of preferring $y_i$ over $y_j$ for a given prompt $x$ is given by
\begin{equation}\label{eq:btm}
    \bigprob(y_i \succ y_j|x) = \frac{p(R_{xy_i}=1|x,y_i)}{p(R_{xy_i}=1|x,y_i) + p(R_{xy_j}=1|x,y_j)}
\end{equation}
During training, the Bradley-Terry preference model is parameterized as follows:
\begin{equation}\label{eq:btm_param}
    \bigprob(y_i \succ y_j| x) = \sigma(r(x,y_i) - r(x,y_j))\,
\end{equation}
where $r(x,y)$ is a trainable function known as the reward function. The resultant maximum likelihood objective is maximized on all $(x,y_i, y_j)$ present in the training data for preference modelling.

Let $r_\text{mle}$ be the maximum likelihood estimate. Equating \eqref{eq:btm} and \eqref{eq:btm_param}, the maximum likelihood estimate of the log-odds is given by
\begin{equation}\label{eq:btm_equate}
    \left. \log \frac{p(R_{xy_i}=1|x,y_i)}{p(R_{xy_j}=1|x,y_j)} \right|_{\text{mle}} = r_\text{mle}(x,y_i) - r_\text{mle}(x,y_j)
\end{equation}

In the rest of the paper, we assume that the trained reward function is already provided to us. For notational convenience, we will drop the $_\text{mle}$ subscript from the rest of the paper.

The proposition below provides an easily-computable form for the importance weighted objective \eqref{eq:approx_is}.
\begin{proposition}
    For the Bradley-Terry preference model defined in \eqref{eq:btm} and parameterized by \eqref{eq:btm_param}, the importance-weighted objective  $\hat{\mathcal{L}_x}(\theta)$ has the following form
    \begin{align}\label{eq:imp_weighted_gen}
        %\hat{\mathcal{L}_x}(\theta) = \sum_{i=1}^n \frac{\exp(r(x,y_i) + \log p(y_i|x) - \log q'(y_i|x))}{\sum_{j=1}^n \exp(r(x, y_j) + \log p(y_j|x) - \log q'(y_j|x))} \log q_\theta (y_i|x)
        & \hat{\mathcal{L}_x}(\theta) = \sum_{i=1}^n \frac{S_i}{\sum_{j=1}^n S_j} \log q_\theta (y_i|x)  \text{ where}  \notag \\ 
        &S_i = \exp(r(x,y_i) + \log p(y_i|x) - \log q'(y_i|x))    
    \end{align}
    
    In the special case where the proposal distribution $q'(y|x)$ is the same as the base distribution $p(y\mid x)$, the importance-weighted objective reduces to
    \begin{equation}\label{eq:imp_weighted_sp}
        \hat{\mathcal{L}_x}(\theta) = \sum_{i=1}^n \frac{\exp(r(x,y_i))}{\sum_{j=1}^n \exp(r(x, y_j))} \log q_\theta (y_i|x)
    \end{equation}
\end{proposition}
\begin{proof}
Lets derive the result for the special case where the proposal distribution $q'(y|x)$ is the same as the base distribution $p(y|x)$. The general case can be derived similarly.
\begin{align}\label{eq:alpha_base}
    \frac{\alpha_i}{\sum_{j=1}^n \alpha_j} &= \frac{p(y_i|x, R_{xy_i}=1)/p(y_i|x)}{\sum_{j=1}^n p(y_j|x, R_{xy_j}=1)/p(y_j|x)}\\
    &= \frac{p(R_{xy_i}=1|x, y_i)/p(R_x=1|x)}{\sum_{j=1}^n p(R_{xy_j}=1|x,y_j)/p(R_x=1|x)} \label{eq:apply_bayes}\\
    &= \frac{p(R_{xy_i}=1|y_i,x)}{\sum_{j=1}^n p(R_{xy_j}=1|y_j, x)} \\
    &=  \frac{1}{\sum_{j=1}^n p(R_{xy_j}=1|y_j, x)/p(R_{xy_i}=1|y_i,x)} \\
    &= \frac{1}{\sum_{j=1}^n  \exp (r(x, y_j) - r(x, y_i))} \label{eq:apply_btm}\\
    &= \frac{\exp(r(x, y_i))}{\sum_{j=1}^n  \exp (r(x, y_j))}
\end{align}
Here \eqref{eq:apply_bayes} follows by applying Bayes rule (see \eqref{eq:posterior}) while \eqref{eq:apply_btm} follows from the Bradley-Terry formulation in \eqref{eq:btm_equate}.
\end{proof}

\subsection{DPO as a special case}
Finally, we we derive the DPO objective as a special case of our baseline-subtracted posterior distillation approach. Specifically, lets impose the following restrictions on our training objective.
\begin{enumerate}
    \item The outputs $y$'s are sampled from the base model, that is, $q'(y|x) = p(y|x)$
    \item For a given prompt $x$, only $2$ outputs are sampled at a time $y_w$ and $y_\ell$. 
    \item The difference between the rewards of the two outputs is very high. Without loss of generality, let $r(x,y_w) \gg r(x,y_\ell)$.
\end{enumerate}
Let $(\alpha_w, \alpha_\ell)$ and $(\beta_w, \beta_\ell)$ represent the importance weights of the samples as defined in \eqref{eq:approx_is_bs}. The first step is to get rid of the reward function from the objective. Based on the above three restrictions, the importance weights can be written as:
\begin{align}
    \frac{\alpha_w}{\alpha_w + \alpha_\ell} & = \frac{\exp(r(x,y_w))}{\exp(r(x,y_w)) + \exp(r(x,y_\ell))} \\
    & = \frac{1}{1 + \exp(r(x,y_\ell) - r(x, y_w))} \approx \frac{1}{1+0} = 1 
\end{align}
Here, the first equation follows from \eqref{eq:alpha_base} since the base model is used as the proposal. The last approximation follows from the third restriction, that is, the reward of the first output is much greater than the reward of the second output. Similarly, one can show that $\frac{\alpha_\ell}{\alpha_w + \alpha_\ell} \approx 0$.

The importance weights of the baseline can be written as
\begin{align}
    & \frac{\beta_w}{\beta_w + \beta_\ell} = \frac{\beta_w/\beta_\ell}{\beta_w/\beta_\ell + 1} \\ \notag
    & = \frac{\exp(\log \beta_w - \log \beta_\ell)}{\exp(\log \beta_w - \log \beta_\ell) + 1} = \sigma(\log \beta_w - \log \beta_\ell)
\end{align}
Similarly, $\frac{\beta_\ell}{\beta_w + \beta_\ell} =  \sigma(\log \beta_\ell - \log \beta_w)$
By incorporating these restrictions in our baseline-subtracted importance sampling gradient estimate \eqref{eq:approx_is_bs}, we get
\begin{align}
    \nabla_\theta \hat{\mathcal{L}_x}(\theta) & \approx \left(1-\frac{\beta_w}{\beta_w + \beta_\ell}\right) \nabla_\theta \log q_\theta(y_w|x) + \left(0 - \frac{\beta_\ell}{\beta_w + \beta_\ell} \right) \nabla_\theta \log q_\theta(y_\ell|x) \\
    & = \frac{\beta_\ell}{\beta_w + \beta_\ell} ( \nabla_\theta\log q_\theta(y_w|x) -  \nabla_\theta q_\theta(y_\ell|x) ) \\
    & = \sigma(\log \beta_\ell - \log \beta_w) ( \nabla_\theta\log q_\theta(y_w|x) -  \nabla_\theta q_\theta(y_\ell|x) ) \\
    & = \sigma\left(\log \frac{q_\theta(y_\ell|x)}{p(y_\ell|x)} - \log \frac{q_\theta(y_w|x)}{p(y_w|x)}\right) ( \nabla_\theta\log q_\theta(y_w|x) -  \nabla_\theta q_\theta(y_\ell|x) )
    \label{eq:dpo_grad}
\end{align}
As shown in \cite{rafailov2023direct}, \eqref{eq:dpo_grad} corresponds to the gradient of the DPO objective when the temperature parameter is set to 1. 

% The optimal policy in DPO satisfies
% \begin{equation}
%     \mathbb{P}(y_1\succ y_2|x) = \sigma(\log \left(\frac{q_\theta(y_1|x)}{p(y_1|x)} - \frac{q_\theta(y_2|x)}{p(y_2|x)})\right)
% \end{equation}
% The PPO-optimal policy for a Bradley-Terry reward model also achieves the same.
% If we can show that there is a unique policy that can achieve the above equation, this will imply that DPO-optimal policy is also the PPO-optimal policy for a Bradley-Terry model

% Let $y_1, \ldots, y_n$ be n samples from $p*(y|x)$ where $p*$ is the optimal distribution of PPO. Let $p(y|x)$ be the base model and $q_\theta(y|x)$ be the training policy. Then the following baseline-subtracted importance sampling approximation will work.
% \begin{equation}
%     \sum_{i=1}^n \left(1/n - \frac{\exp(-r(x,y_i) + \log q_\theta(y_i|x) -\log p(y_i|x))}{\sum_{j=1}^n \exp(-r(x,y_j) + \log q_\theta(y_j|x) -\log p(y_j|x))}\right)\nabla_\theta \log q_\theta(y_i|x)
% \end{equation}
Thus, the above results show that DPO can be derived as a special case of reward-conditioned distillation with baseline-subtraction and self-normalized importance sampling.
% Finally, it is worthy to note that self-normalized importance sampling is biased, and hence, training using the gradient estimate provided in \eqref{eq:approx_is_bs} results in convergence to a different objective as shown in the following proposition:% Rewriting the expected gradient in terms of the proposal distribution $q'(y|x)$, we get
% \begin{equation}
%     \nabla_\theta \mathcal{L}_x(\theta) =  E_{q'(y|x)} \frac{p(y|x, R_{xy}=1)}{q'(y|x)} \nabla_\theta \log q_\theta(y|x)
% \end{equation}
% To obtain a baseline for the above expected gradient, we first note the following
% \begin{align}
%      E_{q'(y|x)} & \frac{q_\theta(y|x)}{q'(y|x)} \nabla_\theta \log q_\theta(y|x) = \sum_{y \in \yset} q'(y|x) \frac{q_\theta(y|x)}{q'(y|x)} \frac{\nabla_\theta q_\theta(y|x)}{q_\theta(y|x)} \\
%      &=\sum_{y \in \yset} \nabla_\theta q_\theta(y|x) 
%      = \nabla_\theta \sum_{y \in \yset} q_\theta(y|x) 
%      = \nabla_\theta 1 = 0
% \end{align}

% Hence, we propose the following baseline for computing the expected gradient:
% \begin{equation}
%     \nabla_\theta \mathcal{L}_x(\theta) = 
% \end{equation}

% Given a reward function $f^*$, input $x$, and two outputs $y_1$ and $y_2$, the probability of preferring $y_1$ over $y_2$ in a Bradley-Terry preference model has the form
% \begin{equation}
%     P(y_1 \succ y_2|x) = \sigma(f^*(x,y_1) - f^*(x,y_2))
% \end{equation}
% Conversely, the log-odds of preferring $y_1$ over $y_2$ can be written as
% In standard preference model training of LLMs, the samples $y$ come from a policy distribution often, denoted here as $p(y \mid x)$. Lets make the following assumptions:
% \begin{enumerate}
%     \item The sample space of $p(y \mid x)$ is finite. For LLMs, this can be imposed by truncating all outputs above a certain length $L$.
%     \item $p(y \mid x) > 0$ for all samples $y$ with length $\le L$.
%     \item Given two samples $y_i$ and $y_j$ from $p(y \mid x)$, $y_i$ is preferred over $y_j$ as follows:
%     \begin{equation}
%             P(y_i \succ y_j|x) = \frac{p(r=1 \mid y_i,x)}{p(r=1 \mid y_i,x) + p(r=1 \mid y_j,x)}
%     \end{equation}
% \end{enumerate}
% Thus, the preference model is a Bradley-Terry model. The prefxxerence probabilities can be approximated by maximizing the following objective over preference pairs:
% \begin{equation}\label{convergence}
%     \mathcal{L}_x(\theta, x) = \sum_{y_i \succ y_j} \log \sigma (f_\theta(x, y_i) - f_\theta(x, y_j)) \,,
% \end{equation}
% where $f_\theta(x,y)$ is a trainable function known as the reward function.

% As the sample size approach infinity and $f$ is flexible enough, the maximum likelihood estimate (MLE) converges.
% \begin{equation}
%     \frac{p(r=1 \mid y_i,x)}{p(r=1 \mid y_j,x)} \approx \exp (f_\mle(x, y_i) - f_\mle(x, y_j))
% \end{equation}




% \subsection{A contrastive approximation to the objective}
% Alternatively, let $q_r'(y|x)$ be a proposal distribution from which we can more easily sample. We can reformulate the objective in \eqref{objective} as follows:
% \begin{align}
%     \mathcal{L}_x &=  E_{p(y \mid x, r)}  \left[ \log q_\theta(y \mid x,r) \right] \\
%     &= E_{p(y \mid x, r)} \left[ \log \frac{q_\theta(y \mid x,r)}{1} \right] \\
%     &= E_{p(y \mid x, r)}\left[ \log \frac{q_\theta(y \mid x,r)}{E_{q_\theta(y \mid x)} 1} \right] \\
%     &= E_{p(y \mid x, r)}\frac{p(r|y,x)}{p(r|x)} \left[ \log \frac{q_\theta(y \mid x,r)}{E_{q_\theta(y \mid x)} 1} \right] \\    
%     &= E_{q_r'(y \mid x)} \frac{p(y \mid x)}{q_r'(y \mid x)} \frac{p(r|y,x)}{E_{p(y|x)}p(r|y,x)} \left[ \log \frac{q_\theta(y \mid x,r)}{E_{q_\theta(y \mid x)} 1} \right] \\    
% \end{align}


% \subsection{Encouraging competition among the sampled outputs}
% Unlike DPO and PPO, the objective defined in \eqref{approx_is} never explicitly attempts to decrease the probability of the low-reward samples. As we show in our experiments in Section~\ref{sec:ablation}, such training can cause the probability of even the low reward samples to increase, which is undesirable. Ideally, we would like that probability of the samples with high reward should increase while those with low-reward should decrease.

% To achieve this, we propose a modified objective where instead of optimizing the KL divergence between the posterior and the policy, we compute the normalized posterior and policy and optimize the KL divergence between them. Let $y_1, \ldots, y_n$ be samples from the proposal distribution $q_r'(y|x)$ as described in Section~\ref{sec:approx_is}. The normalized posterior and policy are defined below:
% \begin{align}
%     p^{norm} (y_i|x, r) &= \frac{p(y_i|x, r)/q_r'(y_i|x)}{\sum_{j=1}^n p(y_j|x, r)/q_r'(y_j|x)}  \\
%         \text{ and } 
%     q^{norm}_\theta (y_i|x, r) &= \frac{q_\theta(y_i|x, r)/q_r'(y_i|x)}{\sum_{j=1}^n q_\theta(y_j|x, r)/q_r'(y_j|x)} 
% \end{align}
% As mentioned in \eqref{eq:alpha}, the importance weights $\frac{p(y_i \mid x,r)}{q_r'(y_i \mid x)}$ that correspond to normalized posterior are referred to as $\alpha_{ir}$. We denote the importance weights $\frac{q_\theta(y_i \mid x,r)}{q_r'(y_i \mid x)}$ that correspond to the normalized policy as $\beta_{ir}(\theta)$.

% The sample approximation to KL-divergence between the normalized posterior and policy can then be written as 
% \begin{align}
% \hat{\mathcal{L}_x}_{norm}(\theta) & = \sum_{i=1}^n p^{norm} (y_i|x, r) \log q^{norm}_\theta (y_i|x, r) \\
% & = \sum_{i=1}^n \left(\frac{\alpha_{ir}}{\sum_{j=1}^n\alpha_{jr}} \right)\log \left(\frac{\beta_{ir}(\theta)}{\sum_{j=1}^n \beta_{jr}(\theta)}\right)\label{eq:norml}\,,
% \end{align}
% where $y_1, \ldots, y_n$ are samples from the proposal distribution $q_r'(y|x)$
% In Appendix~\ref{}, we show that as the number of samples $n\to\infty$, optimizing the KL-divergence between the normalized posterior and policy becomes equivalent to optimizing the KL-divergence between original posterior and policy

% So, why does this objective encourage competition between the outputs? To see this, lets compute the gradient of the normalized objective with respect to the paramters $\theta$. Differentiating \eqref{eq:norml} with respect to $\theta$, we get the following:
% \begin{equation}
%     \nabla_\theta\hat{\mathcal{L}_x}_{norm} (\theta) = \sum_{i=1}^n \left(\frac{\alpha_{ir}}{\sum_{j=1}^n\alpha_{jr}} - \frac{\beta_{ir}(\theta)}{\sum_{j=1}^n \beta_{jr}(\theta)} \right) \nabla_\theta \log q_\theta(y_i|x,r)
% \end{equation}
% Intuititively, the above equation states that if the posterior assign higher normalized importance weight to a sampled output $y_i$ than the policy, the difference between the normalized importance weights is positive and hence, the policy is trained to increase the log-probability of that output.

% On the other hand, if the posterior assigns lower normalized importance weight to an output than the policy, the difference is negative and hence the policy is trained to decrease the log-probability of that output.

% The model converges when the policy learns to assign the same normalized importance weight to the outputs as the posterior. Notably, the policy is forced to follow the same ratio of 

% \subsection{Choosing an Effective Proposal Distribution}

% The effectiveness of importance sampling hinges on the choice of the proposal distribution $q'(y|x, r)$. Ideally, this distribution should be:
% \begin{enumerate}
%     \item \textbf{Easy to Sample From:} $q'(y|x, r)$ should allow for efficient generation of samples.
%     \item \textbf{Similar to the Posterior:} The closer $q'(y|x, r)$ is to $p(y|x,r)$, the lower the variance of the importance sampling estimator will be, leading to more efficient approximations.
% \end{enumerate}
% We consider two proposal distributions: the prior $p(y|x)$ and the trainable approximate posterior from a previous time-step $q_\theta^{(t)}(y|x,r)$.

% \subsubsection{Prior as proposal distribution}
% When $p(y|x)$ is used as the proposal, the fraction $\frac{\alpha_i^r}{\sum_{j=1}^n \alpha_j^r}$ can be written as
% \begin{align}
%      \frac{\alpha_i^r}{\sum_{j=1}^n \alpha_j^r} &= \frac{p(y_i|x,r)/p(y_i|x)}{\sum_{j=1}^n p(y_j|x,r)/p(y_j|x)} 
% \end{align}
% From the Bayes' formulation in \eqref{posterior}, the ratio between the posterior and prior can be written as the ratio between the reward distributions $p(r|y,x)$ and $p(r|x)$.
% \begin{align}
%      \frac{\alpha_i^r}{\sum_{j=1}^n \alpha_j^r} &= \frac{p(r|y_i,x)/p(r|x)}{\sum_{j=1}^n p(r|y_j, x)/p(r|x)} \\
%      &= \frac{p(r|y_i,x)}{\sum_{j=1}^n p(r|y_j, x)}
% \end{align}

% \subsubsection{Approximate posterior as proposal distribution}
% When $q_\theta^(t)(y|x, r)$ is used as the proposal, the fraction $\frac{\alpha_i^r}{\sum_{j=1}^n \alpha_j^r}$ can be written as
% \begin{align}
%      \frac{\alpha_i^r}{\sum_{j=1}^n \alpha_j^r} &= \frac{p(y_i|x,r)/q_\theta^(t)(y_i|x,r)}{\sum_{j=1}^n p(y_j|x,r)/q_\theta^(t)(y_j|x, r)} \\
%      &= \frac{\left(p(y_i|x)/q_\theta^(t)(y_i|x,r)\right) * \left(p(r|y_i,x)/p(r|x)\right)}{\sum_{j=1}^n \left(p(y_j|x)/q_\theta^(t)(y_j|x,r)\right) * \left(p(r|y_j,x)/p(r|x)\right)} \\
%      &= \frac{p(r|y_i,x)*\left(\frac{p(y_i|x)}{q_\theta^(t)(y_i|x,r)}\right) }{\sum_{j=1}^n p(r|y_j,x) * \left(\frac{p(y_j|x)}{q_\theta^(t)(y_j|x,r)} \right)} \\
% \end{align}

% As long as we can compute the importance weights $\frac{p(r \mid y,x)}{p(r \mid x)}$, the above objective can easily by approximated using Monte Carlo techniques. 

% \section{The Importance Weights}
% \subsection{Bradley-Terry model}
% Consider a finite set of samples denoted as $\{y_1, \ldots, y_n\}$, each associated with a corresponding set of probabilities $\{p_1, \ldots, p_n\}$. The model defines the probability of preferring a sample $y_i$ over $y_j$ as follows:

% \begin{equation}
%     P(y_i \succ y_j) = \frac{p_i}{p_i + p_j}
% \end{equation}

% Introducing a parametric representation, let $\frac{p_i}{p_j}$ be expressed as $\exp (f_\theta(y_i) - f_\theta(y_j))$, where $f_\theta$ is a parameterized function. Under this representation, the maximum likelihood objective for a sequence of preference pairs $(y_i, y_j)$ is formulated as:

% \begin{equation}
%     \mathcal{L}_x(\theta) = \sum_{y_i \succ y_j} \log \sigma (f_\theta(y_i) - f_\theta(y_j))
% \end{equation}

% As the sample size approaches infinity, the Maximum Likelihood Estimate (MLE)  denoted as $f_\mle$, converges.

% \begin{equation}
%     \frac{p_i}{p_j} \approx \exp (f_\mle(y_i) - f_\mle(y_j)) 
% \end{equation}





% \subsection{Computing the importance weights}
% For a given value of reward $r$ and input $x$, the importance weight of an output $y$ will be denoted as $IW(y:x,r)$
% For $r=1$, the importance weight in \eqref{importance} can be written as 
% \begin{equation}
%     IW(y;x,r=1) = \frac{p(r=1 \mid y,x)}{\mathbb{E}_{\bar{y} \sim p(y \mid x)} p(r=1 \mid \bar{y},x)}
% \end{equation}
% Given samples $y_1, \ldots, y_n$ from $p(y \mid x)$, the importance weight can be written as
% \begin{equation}
%    IW(y;x,r=1)= \frac{p(r=1 \mid y,x)}{\frac{1}{n}\sum_{y_j}p(r=1 \mid y_j,x)}
%     = \frac{1}{\frac{1}{n}\sum_{y_j}\frac{p(r=1 \mid y_j,x)}{p(r=1 \mid y,x)}}
% \end{equation}
% Replacing \eqref{convergence}, we get
% \begin{align}
%     IW(y;x,r=1) &\approx \frac{n}{\sum_{y_j} \exp( f_\mle (x,y_j) - f_\mle (x, y))}\\
%     &= \frac{n\exp(f_\mle(x,y))}{\sum_{y_j} \exp( f_\mle (x,y_j))}
% \end{align}
% Unlike the case for $r=1$, there is no straightforward way to compute the importance weight for $r=0$. For the sake of symmetry, we will assume it to be 
% \begin{equation}
%     IW(y;x, r=0) = \frac{n\exp(-f_\mle(x,y))}{\sum_{y_j} \exp( -f_\mle (x,y_j))}
% \end{equation}
% However, please note that this is an assumption in the proposed model and doesn't follow from the Bradley-Terry reward model.
%% Do not delete
% We are interested in distilling the posterior distribution $p(y \mid x, r=1)$. For this we look at Importance Sampling approaches, reparametrizing sampling from the posterior as sampling from $p(y \mid x)$ through the relation

% \begin{equation}
%     p(y \mid x, r=1) = \frac{p(r=1 \mid y, x)}{p(r=1 \mid x)} p(y \mid x)
% \end{equation}

% \noindent and using the relation

% \begin{equation}
%     \frac{p(r=1 \mid y, x)}{p(r=1 \mid x)} = \frac{\exp(R_1(x, y))}{\sum_{y' \in D_y} \exp(R_1(x, y'))}
% \end{equation}

% \noindent where $p(r=1 \mid y, x)$ is defined as

% \begin{equation}
%     p(r=1 \mid y, x) = \frac{\exp(R_1(x, y))}{\exp(R_1(x, y)) + \exp(R_0(x, y))}
% \end{equation}

% \noindent and

% \begin{equation}
%     p(r=1 \mid x) = \sum_{y' \in D_y} p(r=1 \mid y', x)p(y' \mid x) 
% \end{equation}
%%

% \begin{align*}
% P(i \text{ preferred over } j) &= \frac{\exp(f_i)}{\exp(f_i) + \exp(f_j)} \\
% f(y_i \succ y_j; \theta) &= \exp\left\{ \eta(\theta) 1\{y_i \succ y_j\} - A(\theta) \right\} \\
% \text{where} \quad \eta(\theta) &= f_i - f_j, \\  \quad A(\theta) &= \log(1 + \exp(f_i-f_j))
% \end{align*}

% \subsection{Direct Posterior Sampling}

% Using the probability ratio parametrization, one can directly express the posterior as

% \begin{align*}
%     p(y \mid x, r=1) &= \frac{p(r=1 \mid y, x)p(y \mid x)}{\sum_{y' \in V^*} p(r=1 \mid y',x)p(y' \mid x)}\\
%                      &= \frac{p(y \mid x)}{\sum_{y' \in V^*} \frac{p(r=1 \mid y',x)}{p(r=1 \mid y',x)} p(y' \mid x)}\\
%                      &= \frac{p(y \mid x)}{\sum_{y' \in V^*} \exp(f_\mle(x, y') - f_\mle(x, y)) \exp(\log p(y' \mid x)}\\
%                      &= \frac{p(y \mid x)}{\sum_{y' \in V^*} \exp(f_\mle(x, y') + \log p(y' \mid x) - f_\mle(x, y))}\\
%                      &= \frac{\exp(f_\mle(x, y) + \log p(y \mid x)))}{\sum_{y' \in V^*} \exp(f_\mle(x, y') + \log p(y' \mid x))}
% \end{align*}

% where $V*$ is the set of all strings made of words of a vocabulary $V$.
% Unfortunately it is impossible to sample from this distribution, due to its intractable
% partition function, but we had the same problem before, so we could try to
% approximate with samples $\mathcal{Y} = \{ y_1 \cdots y_n : y_j \sim p(y \mid
% x)\}$ and use perturb and map

% \begin{equation}
% j \sim \arg\max \left\{ \begin{bmatrix}
% f_\mle(x, y_1) + \log p(y_1 \mid x) + \Gamma_1 \\
% \cdots \\
% f_\mle(x, y_n) + \log p(y_n \mid x) + \Gamma_n \\
% \end{bmatrix}\right\}
% \end{equation}

% \noindent to get

% \begin{equation}
% \mathcal{Y}_j \sim p(y \mid x, r=1)
% \end{equation}

% Here $\Gamma_j$ are samples from Gumbel noise. Probably there are better way to sample, Metropolis Hastings?


% \newpage
% Given samples \( y_1, y_2, \ldots, y_n \) from \( p(y|x) \), we aim to estimate the expectation of \( \log q(y|x,r=1) \) under the distribution \( \frac{p(y|x)p(r=1|y,x)}{\sum_{y'}p(y'|x)p(r=1|y',x)} \). Let $\mathcal{Y}$ be the sample space of $p(y|x)$. The steps are as follows:

% \begin{enumerate}
%     \item  Generate \( n \) independent samples \( y_1, y_2, \ldots, y_n \) from the distribution \( p(y|x) \).
%     \item  For each sample \( y_i \), compute \( p(r=1|y_i,x) \).
%     \item Estimate the normalization constant \( C_n \) using the samples. It is approximated as:
%     $ C_n \approx \frac{1}{n} \sum_{i=1}^{n} p(r=1|y_i,x) $
%     \item Calculate the weighted average of \( \log q(y_i|x,r=1) \) values as an estimate of the expected value:
%     $ \hat{E}_n = \frac{1}{n} \sum_{i=1}^{n} \frac{p(r=1|y_i,x)}{C_n} \log q(y_i|x,r=1) $
% \end{enumerate}

% \textbf{Proof of Convergence:}

% To prove that this method is consistent, we show that as \( n \rightarrow \infty \), \( \hat{E}_n \) converges to the true expectation of \( \log q(y|x,r=1) \) under the modified distribution.

% \begin{enumerate}
%     \item \textbf{Consistency of the Normalization Constant:} By the Law of Large Numbers (LLN), we have:
%      $$C_n = \frac{1}{n} \sum_{i=1}^{n} p(r=1|y_i,x) \xrightarrow{p} E_{p(y|x)}[p(r=1|y,x)] $$
%     as \( n \rightarrow \infty \).

%     \item \textbf{Consistency of the Weighted Average:} Given the consistency of \( C_n \), substituting it into the expectation we get
%     \begin{align}
%         & \frac{1}{n} \sum_{i=1}^{n} \frac{p(r=1|y_i,x)}{C_n} \log q(y_i|x,r=1) \\
%         & = \frac{1}{{E_{p(y|x)}[p(r=1|y,x)]}}\frac{1}{n} \sum_{i=1}^{n} p(r=1|y_i,x)\log q(y_i|x,r=1)
%         & = 
%     \end{align}
    
%     Applying the LLN again, we have:
%     \begin{align}
%         &\frac{1}{{E_{p(y|x)}[p(r=1|y,x)]}}\frac{1}{n} \sum_{i=1}^{n} p(r=1|y_i,x)\log q(y_i|x,r=1) \\
%         & \xrightarrow{p}  \frac{1}{{E_{p(y|x)]}[p(r=1|y,x)]}} E_{p(y|x)}[p(r=1|y,x)\log q(y_i|x,r=1)] \\
%         &= \frac{E_{p(y|x)}[p(r=1|y,x)\log q(y|x,r=1)]}{{E_{p(y|x)]}[p(r=1|y,x)]}} \\
%         &= \sum_{y} \left(\frac{p(y|x)p(r=1|y,x)}{\sum_{y'}p(y'|x)p(r=1|y',x)}\right)\log q(y'|x,r=1)
%     \end{align}
%     as \( n \rightarrow \infty \).
% \end{enumerate}

% Therefore, the method is consistent, and the estimate converges to the true expectation as \( n \rightarrow \infty \).


